Long- and short-range correlations and their event-scale dependence in high-multiplicity pp collisions at $\boldsymbol{\sqrt{{\textit s}}}=13$ TeV

Two-particle angular correlations are measured in high-multiplicity proton-proton collisions at $\sqrt{s} =13$ TeV by the ALICE Collaboration. The yields of particle pairs at short-($\Delta\eta$ $\sim$ 0) and long-range ($1.6 < |\Delta\eta| < 1.8$) in pseudorapidity are extracted on the near-side ($\Delta\varphi$ $\sim$ 0). They are reported as a function of transverse momentum ($p_{\mathrm T}$) in the range $1 <p_{\mathrm T}< 4$ GeV/$c$. Furthermore, the event-scale dependence is studied for the first time by requiring the presence of high-$p_{\rm T}$ leading particles and jets for varying $p_{\rm T}$ thresholds. The results demonstrate that the long-range "ridge" yield, possibly related to the collective behavior of the system, is present in events with high-$p_{\mathrm T}$ processes. The magnitudes of the short- and long-range yields are found to grow with the event scale. The results are compared to EPOS LHC and PYTHIA 8 calculations, with and without string-shoving interactions. It is found that while both models describe the qualitative trends in the data, calculations from EPOS LHC show a better quantitative agreement, in particular for the $p_{\rm T}$ and event-scale dependencies.

==> abstract.tex <==
We report on the studies of two-particle angular correlations measured in high-multiplicity proton-proton collisions at $\sqrt{s} =13$ TeV with ALICE. 
The yields of two-particle angular correlations at short-($\Delta\eta$ $\sim$ 0) and long-range ($1.6 < |\Delta\eta| < 1.8$) in rapidity are measured at the near side ($\Delta\varphi \sim 0$).
The correlations and yields are reported as a function of charged-particle transverse momentum ($p_{\mathrm T}$) in $1 < p_{\mathrm T} < 5$ GeV/$c$.
Furthermore, the event-scale dependence has for the first time been studied by requiring the presence of high-$p_{\rm T}$ leading tracks and/or jets for varying $p_{\rm T}$ thresholds. 
The results demonstrate that the long-range ``ridge`` yield, related to the collective behavior of the produced system, is present in events with high-$p_{\mathrm T}$ processes. The magnitudes of the short- and long-range yields are found to grow with the event scale. 
The results have been compared to calculations with EPOS LHC and PYTHIA 8, with and without string-shoving interactions. It is found that while both models describe the qualitative trends in the data, EPOS LHC shows a better quantitative agreement, in particular for the $p_{\rm T}$ and event scale dependences.

